IPoD: Implicit Field Learning with Point Diffusion for Generalizable 3D Object Reconstruction from Single RGB-D Images

Generalizable 3D object reconstruction from single-view RGB-D images remains a challenging task, particularly with real-world data. Current state-of-the-art methods develop Transformer-based implicit field learning, necessitating an intensive learning paradigm that requires dense query-supervision uniformly sampled throughout the entire space. We propose a novel approach, IPoD, which harmonizes implicit field learning with point diffusion. This approach treats the query points for implicit field learning as a noisy point cloud for iterative denoising, allowing for their dynamic adaptation to the target object shape. Such adaptive query points harness diffusion learning's capability for coarse shape recovery and also enhances the implicit representation's ability to delineate finer details. Besides, an additional self-conditioning mechanism is designed to use implicit predictions as the guidance of diffusion learning, leading to a cooperative system. Experiments conducted on the CO3D-v2 dataset affirm the superiority of IPoD, achieving 7.8% improvement in F-score and 28.6% in Chamfer distance over existing methods. The generalizability of IPoD is also demonstrated on the MVImgNet dataset. Our project page is at https://yushuang-wu.github.io/IPoD.

==> tables/alg.tex <==
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}[t]
\caption{Self-conditioning.}
\label{alg:self_cond}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]
# Algorithm in a Pytorch-like style:
# B, N: batch size, point number;
# I, P, X_0, X_t, t: variables as in paper;
# udf, eps: implicit value and noise prediction;
# foward(): function of model forward;
# update(): function of X_t updating.

def train(I, P, X_0): # for the training stage
    ... # prepare t, X_t and supervision
    self_cond = torch.zeros([B, N, 1]) - 1
    
    if random.choice([0, 1]) > 0.5:
        udf, eps = foward(I, P, X_t, t, self_cond)
        self_cond = udf.detach()
        
    udf, eps = foward(I, P, X_t, t, self_cond)
    ... # compute loss
    
    
def infer(I, P): # for the inference stage
    self_cond = torch.zeros([B, N, 1]) - 1
    X_t = torch.randn([B, N, 3])
    
    for t in reversed(range(T)): 
        udf, eps = foward(I, P, X_t, t, self_cond)
        self_cond = udf        # update self-condition
        X_t = update(X_t, eps) # update X_t
        
    return X_t
\end{lstlisting}
\end{algorithm}


==> tables/equations.tex <==
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\point}{\boldsymbol{x}}

%\resizebox{0.48\textwidth}{!}{
    %\large
\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llll}
        \toprule
        Notation & Example\\
        \midrule
         Fraction &  $\frac{1}{a}$ \\
         Max & $\max (a, 0 )$ \\
         Dimension & $\boldsymbol{x} \in \mathbb{R}^3$ \\
         Argmax  & $\mathop{\arg\max}_{a} f(ax)$ \\
         cos & $\cos(x)$ \\
         Hat/tilde & $\hat{\boldsymbol{x}}, \tilde{\boldsymbol{x}}$ \\
         Tensor operation & $\otimes$, \quad $\circ$, \quad $\odot$ \\ 
         Sum & $\sum_{i=1}^{N} x_i$ \\
         Approximation & $f(x) \approx g(x)$ \\
         Around & $\sim$100 \\
         Product & $\prod_{i=1}^{N} x_i$ \\
         Integral & $\int_{-\infty}^{+\infty} x_i$ \\
         Gradient & $\boldsymbol{n}(n) = \nabla o(\boldsymbol{x})/\|\nabla o(\boldsymbol{x})\|_2$ \\
         Parallel & $\mathcal{L} = \sum \| x_i - \hat{x}_i \|^2_2$ \\
         Set & $\{I_i | i=1,\dots, N \}$ \\
        \bottomrule
    \end{tabular}
%    }



==> tables/greek_letters.tex <==
    \resizebox{0.48\textwidth}{!}{
    \large
    \begin{tabular}{clclclclc}
        \toprule
        Symbol & \LaTeX  & Symbol & \LaTeX & Symbol & \LaTeX\\
        \midrule
$\alpha  $ & \textbackslash alpha   & $\kappa $ & \textbackslash kappa  & $\psi    $  & \textbackslash psi    \\
$\beta   $ & \textbackslash beta    & $\lambda$ & \textbackslash lambda & $\rho    $  & \textbackslash rho    \\
$\chi    $ & \textbackslash chi     & $\mu    $ & \textbackslash mu     & $\sigma  $  & \textbackslash sigma  \\
$\delta  $ & \textbackslash delta   & $\nu    $ & \textbackslash nu     & $\tau    $  & \textbackslash tau    \\
$\epsilon$ & \textbackslash epsilon & $ o     $ & \textbackslash o      & $\theta  $  & \textbackslash theta  \\
$\eta    $ & \textbackslash eta     & $\omega $ & \textbackslash omega  & $\upsilon$  & \textbackslash upsilon\\
$\gamma  $ & \textbackslash gamma   & $\phi   $ & \textbackslash phi    & $\xi     $  & \textbackslash xi     \\
$\iota   $ & \textbackslash iota    & $\pi    $ & \textbackslash pi     & $\zeta   $  & \textbackslash zeta   \\
\midrule
$ \digamma   $ & \textbackslash digamma    & $ \Delta $ & \textbackslash digamma    & $ \Theta   $  & \textbackslash Theta  \\
$ \varepsilon$ & \textbackslash varepsilon & $ \Gamma $ & \textbackslash varepsilon & $ \Upsilon $  & \textbackslash Upsilon\\
$ \varkappa  $ & \textbackslash varkappa   & $ \Lambda$ & \textbackslash varkappa   & $ \Xi      $  & \textbackslash Xi     \\
$ \varphi    $ & \textbackslash varphi     & $ \Omega $ & \textbackslash varphi     &               &         \\
$ \varpi     $ & \textbackslash varpi      & $ \Phi   $ & \textbackslash varpi      & $ \aleph   $  & \textbackslash aleph  \\
$ \varrho    $ & \textbackslash varrho     & $ \Pi    $ & \textbackslash varrho     & $ \beth    $  & \textbackslash beth   \\
$ \varsigma  $ & \textbackslash varsigma   & $ \Psi   $ & \textbackslash varsigma   & $ \daleth  $  & \textbackslash daleth \\
$ \vartheta  $ & \textbackslash vartheta   & $ \Sigma $ & \textbackslash vartheta   & $ \gimel   $  & \textbackslash gimel  \\
        \bottomrule
    \end{tabular}
    }



==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

